SPARTA: A Divide and Conquer Approach to Address Translation for Accelerators

Virtual memory (VM) is critical to the usability and programmability of hardware accelerators. Unfortunately, implementing accelerator VM efficiently is challenging because the area and power constraints make it difficult to employ the large multi-level TLBs used in general-purpose CPUs. Recent research proposals advocate a number of restrictions on virtual-to-physical address mappings in order to reduce the TLB size or increase its reach. However, such restrictions are unattractive because they forgo many of the original benefits of traditional VM, such as demand paging and copy-on-write. We propose SPARTA, a divide and conquer approach to address translation. SPARTA splits the address translation into accelerator-side and memory-side parts. The accelerator-side translation hardware consists of a tiny TLB covering only the accelerator's cache hierarchy (if any), while the translation for main memory accesses is performed by shared memory-side TLBs. Performing the translation for memory accesses on the memory side allows SPARTA to overlap data fetch with translation, and avoids the replication of TLB entries for data shared among accelerators. To further improve the performance and efficiency of the memory-side translation, SPARTA logically partitions the memory space, delegating translation to small and efficient per-partition translation hardware. Our evaluation on index-traversal accelerators shows that SPARTA virtually eliminates translation overhead, reducing it by over 30x on average (up to 47x) and improving performance by 57%. At the same time, SPARTA requires minimal accelerator-side translation hardware, reduces the total number of TLB entries in the system, gracefully scales with memory size, and preserves all key VM functionalities.

==> tex/design.tex <==
\section{SPARTA}
\label{sec:msmmu}

\javier{Points to come across:

\begin{itemize}
  \item Implementation and how it tackles the TLB reach and penalty.
  \item We need figures explaining how the translation works with steps. 
\end{itemize}

}

In this section, we investigate the design space for address translation for MPUs, given the modest associativity requirements and the characteristics of our memory-chip network. Then, we propose and describe our solution, SPARTA.

\subsection{Placement}

A straightforward extension of address translation to MPUs integrates an MMU in each MPU. Each MPU probes its MMU on each memory access, and upon a miss in its TLBs, initiates a conventional page table walk. Fig.~\ref{fig:baseline} shows a page walk that references a page table entry residing in another memory chip and partition, which is the common case in systems with multiple chips and partitions. Blue arrows indicate translation-related memory messages, while red arrows show data fetch. %In other words, memory accesses to page table entries are colored in blue, while accesses to page frames are red. 

\input{tex/float-translation-schemes}

There are several problems with this baseline. First, the page table entry that contains the physical address can be anywhere in the system, involving expensive interconnect traversals which makes page walks costly. Second, the data fetch cannot begin until the translation operation finishes, adding the translation latency to the data fetch latency. Third, the translation process does not finish until the page table entry returns to the MPU, even if the page table entry and the target page frame are in the same chip or memory partition. The fundamental problem is that there is no direct relation between virtual page numbers and page frames, something inherent to fully associative VM. The consequence is that there is no expected correlation between the location of page table entries and page frames, precluding fetching the data before the page table entry returns to the MPU. Although this design makes sense for fully associative VM, it is not optimal for set-associative VM.

We now exploit the modest associativity requirements and consider memory sets that span a memory chip only. A virtual address identifies a memory chip uniquely, and hence we know that the target page frame is somewhere in that chip. Under this constraint, we can utilize a centralized per-chip MMU, along with a page table and a set of TLBs, as shown in Fig.~\ref{fig:chipmmu}. Upon a page walk operation from an MPU, the virtual address is used to access the per-chip MMU. If the translation is not in the per-chip TLBs, a page walk in the memory chip begins. When the page walk finishes, the MMU in the memory chip starts the data fetch immediately, referencing the page frame (which can reside in any of the partitions in the chip). When the data returns to the per-chip MMU, both the page table entry and data return to the MPU. 

This method is an improvement over the baseline for two reasons. First, translation and data fetch overlap the latency on the interconnect to reach the target memory chip, as only the virtual address is used to locate the memory chip. Second, the translation process finishes as soon as the page walk within the memory chip finishes. However, there is room for improvement. As the virtual address only identifies the memory chip, page frames and page table entries can be in any memory partition. This placement creates two problems. First, the centralized per-chip MMU can be located anywhere in the chip, and upon a page walk, the page table entry could be located in a different partition. Second, the target page frame might also be located in another partition. Based on the latency results of Fig.~\ref{fig:e2elat}, the overhead could be significant. 

Going beyond, we can co-locate the page table entries and the page frames in the same memory partition, where memory accesses are faster, and employ a per-partition MMU. In this case, shown in Fig.~\ref{fig:partitionmmu}, memory sets only encompass a memory partition. The locality-aware placement of the MMU delivers the best performance among all. First, the translation and data fetch operations overlap the latency to reach the memory partition---because only the virtual address is used to locate the memory partition. Second, the translation finishes as soon as the page walk within the memory partition finishes, and since the target page frame is within the same partition, the data fetch can begin immediately (without traversing any interconnect).

\subsection{Page Table}
\label{sec:pagetable}

After defining the location of the memory-side MMUs, the next step is to choose a page table. Although there are many page table implementations~\cite{yaniv:hash}, we choose an inverted page table for the following reasons. First, inverted page tables do not need to be dynamically resized, so they are allocated once and pinned contiguously in memory~\cite{jacob:look}. Second, all the processes whose pages map to the partition share the same page table. Finally, when there are no collisions in the inverted page table, page walks only require a single memory access.

One of the key parameters of an inverted page table is the ratio between the number of page frames and page table entries, also called the load factor~\cite{cormen:introduction}. The load factor directly dictates the rate of collisions (i.e., the frequency of two virtual page numbers mapping to the same page table entry). Importantly, given a load factor, the collision rate is not affected by the working set size or access patterns, assuming uniform hashing~\cite{cormen:introduction}. In Fig.~\ref{fig:memref}, we compare a conventional modulo hash to a stronger k-bit XOR folding~\cite{qureshi:fundamental}, to demonstrate the effects of hashing on page table collisions. As we have not seen significant differences in workloads, process counts, and memory size to working set size ratios, we present an average of all the results. The results indicate that an inverted page table with a load factor of $1/4$ and the fold hash function practically removes all collisions. To achieve similar performance with the modulo hash function we would need a load factor of $1/8$. Hence, our design employs an inverted page table with a k-bit XOR folding hash function and load factor of 1/4.  

\begin{figure}
\centering
   \subfloat[\parbox{0.3\columnwidth}{Memory references per page walk.}]{
     \label{fig:memref}
     \includegraphics[width=0.45\columnwidth]{graphs/memrefs-bw.pdf}
   }
   \subfloat[\parbox{0.25\columnwidth}{Page walk latency normalized to DRAM latency.}]{
     \label{fig:pagewalklat}
     \includegraphics[width=0.45\columnwidth]{graphs/pagewalklat-bw.pdf}
   }
   \caption{Inverted page table performance.}
   \label{fig:IPT_perf_load_hash}
\end{figure}

Fig.~\ref{fig:pagewalklat} shows the page walk latency normalized to the latency of a single DRAM access. The page walk latency is within $1.005\times$ of a DRAM access. The reason the page walk latency does not directly correlate with the number of memory references per walk is that we use open addressing for resolving conflicts~\cite{yaniv:hash}. In open addressing, upon a collision, we probe the next entry in the inverted page table, rather than dereferencing a pointer to a new page table entry, exploiting the locality in the DRAM row buffer~\cite{qureshi:fundamental}, and thus reducing the latency overhead of collisions. Additionally, open addressing removes the pointer per page table entry required to resolve collisions. Each entry in our page table holds a 36-bit virtual page number (VPN), a 12-bit address space identifier (ASID), the 36-bit page frame number (PFN),\footnote{Note that we include the PFN and hence support synonyms.} and 12 bits for page flags, fitting in 16-byte entries. We assume 48-bit virtual and physical address. As we allocate four 16B entries for each 4KB page, due to the 1/4 load factor, the inverted page table consumes a modest $1.6\%$ of the physical memory.  

\subsection{TLB Hierarchy}
\label{sec:tlb}

Although a page walk usually introduces a single additional DRAM access within the memory partition, such accesses are still on the critical path. To minimize this overhead, we employ a TLB hierarchy within the memory-side MMUs to cache frequently used translations. Fig.~\ref{fig:tlb_hitratio} shows how the TLB hit ratio scales as the number of entries increases (more details on the methodology are found in Section~\ref{sec:methodology}). As our translation performance is less dependent on the TLB's hit ratio (due to fast page walks), we average the results across all workloads and scenarios. However, because the memory-side MMUs are shared across all processes in the system (in contrast to conventional MMUs which are bound to a single execution unit), we break down the average results across process counts. Although we expect few processes running concurrently on the MPU cluster,\footnote{A single process can run on an arbitrary number of MPUs.} we see that even with 8 different processes, a TLB with 64 entries, which is the usual size of a first-level TLB, achieves a hit ratio in excess of than $80\%$. Additionally, increasing the number of entries beyond 1024 gives diminishing results, which again matches the size of a conventional second-level TLB. Hence, a conventional two-level TLB hierarchy, a first level with 64 entries and a second level with 1024 is a sound approach. As each MMU integrates its own TLBs, its TLB content does not reflect accesses to others partitions and hence is robust across any memory chip and partition counts.

%All MPUs running in the same address space are a single process

\begin{figure}[t]
   \centering
   %\includegraphics[width=0.8\columnwidth]{graphs/tlbhitratio-marker.pdf}
   \includegraphics[width=0.8\columnwidth]{graphs/tlbmissratio.pdf}
   \caption{TLB hit ratio sensitivity analysis.}
   \label{fig:tlb_hitratio}
   
\end{figure}

\begin{figure}
\centering

 \subfloat[TLB hit operation.]{
  \label{fig:tlb_hit}
%  \includegraphics[width=.32\textwidth,clip,trim = 18mm 213mm 117mm 20mm]{figs/eps/sim-rread-lat.eps}}
   \includegraphics[clip,width=0.95\columnwidth]{figures/hit2.pdf}
   }
   
%  \hspace{.01in}

 \subfloat[TLB miss operation.]{
  \label{fig:tlb_miss}
%  \includegraphics[width=.32\textwidth,clip,trim = 18mm 213mm 115mm 20mm]{figs/eps/sim-rread-bw.eps}}
 \includegraphics[clip,width=0.95\columnwidth]{figures/miss2.pdf}
 }

\caption{Operation flow of memory-side MMUs.
 \label{fig:tlb_ops}}
 
\end{figure}

\subsection{Putting Everything Together}
Now that we have defined the placement of the MMUs, the page table, and the TLB hierarchy, we provide a walkthrough of the memory-side MMU's operation in Fig.~\ref{fig:tlb_ops}.

In Fig.~\ref{fig:tlb_hit}, we look at the case where the TLBs in the memory-side MMU experience a hit. A request from an MPU arrives at the router of the target partition which forwards it to the MMU (1). A mux checks whether the message uses virtual or physical addresses (2). Memory requests that use physical addresses either come from CPU cores, DMAs, or MPUs that hit in their TLBs.\footnote{MPUs tag requests that use virtual addresses with a cookie.} In the case of physical addresses, the request is sent directly to the DRAM controller. In this example, the request uses virtual addresses, hence arriving at the MMU, and the TLB hierarchy is probed, resulting in a TLB hit (3). Note that the hit requires both the VPN and ASID bits (which are in the request) to match. The MMU then appends the offset bits to the PFN to generate the physical address, creates an MSHR entry tagged with the physical address, and sends a request to the DRAM controller (4). When the DRAM controller finds the address, it sends DRAM commands to fetch the appropriate cache block (5). When the reply comes back (6), the DRAM controller forwards the reply to the MMU, which checks the MSHRs for a match (7). Upon a match, the MMU sends the reply back to the MPU, containing both the data and translation (8).

In Fig.~\ref{fig:tlb_miss}, the memory-side MMU experiences a miss in its TLBs, triggering a page walk. A virtual request from an MPU arrives at the mux (1) and gets forwarded to the memory-side MMU (2). The MMU probes its TLB hierarchy, but the page table entry is not cached (3). The MMU generates the physical address of the page table entry by adding the output of the hash function on the request's virtual address to the base address of the inverted page table. The MMU then creates an MSHR entry tagged with this physical address and sends the request (for the page table entry) to the DRAM controller (4). When the DRAM controller finds the address, it sends DRAM commands to fetch the appropriate page table entry (5). When the reply comes back (6), the DRAM controller forwards the reply to the MMU. The MMU checks the MSHRs for a match (7). The matching MSHR entry indicates that it was a page walk, and hence the MMU generates the request for the actual cache block (8), and repeats the steps shown for the TLB hit operation: (9), (10), and (11). Last, the MMU sends the reply back to the MPU with the data and translation (12). 

Note that most of the functionality of the MSHRs in the MMU is performed by the request queues at the memory controller. We could extend the state of the queues and provide the same functionality. However, we avoid the complexity of extending the memory controller due to the modest hardware requirements for the MSHRs, 64 to 128 entries~\cite{lee:simultaneous} assuming worst-case overprovisioning. Additionally, to further reduce the already low bandwidth requirements of page walks (due to high TLB hit ratios), we indicate to the memory controller that the request for the page table entry is 16 bytes, instead of the conventional 64-byte requests. Existing memory controllers of 3D memories already support requests of different size~\cite{micron:hmc}.




==> tex/discussion.tex <==
\section{Discussion \& Future Work}
\label{sec:discussion}

Following the prior work, we assumed that the accelerators do not have
caches~\cite{haria:devirtualizing, picorel:near-memory}, as they are
usually tailored for acceleration of data traversals that are not
cache friendly. However, SPARTA is equally applicable to systems with
caches, as well as the systems with execution-side TLBs and MMUs. In
such cases, SPARTA would be very useful in accelerating the handling of
TLB misses. Recent practical designs for virtual cache
hierarchies~\cite{yoon:revisiting, park:efficient,} would also be a
great fit for SPARTA, obviating the need for execution-side TLB
hardware. Also note that SPARTA could be used for accelerating CPU TLB
misses, which we plan to explore in the future.

%\noindent\textbf{Page faults.} Upon a page fault triggered by an MPU, we choose to interrupt the CPU to run a handler, as MPUs may not be capable of running an OS. The memory-side MMU notifies the MPU of the fault, and then the MPU places a request in a memory-mapped queue indicating the faulting virtual address and MPU's id. Then, it raises an interrupt on the CPU. The handler running on the CPU resolves the page fault and updates both the CPU's and memory-side MMU's page table. All MMU state is exposed through memory-mapped IO with an uncacheable memory policy. Once the fault is serviced, the handler notifies the appropriate MMU, which resumes execution and retries the faulting address. Such page fault processing is also employed in today's integrated GPUs~\cite{vesely:observation}.\\

%\noindent\textbf{TLB shootdowns.} Many ways exist to maintain the memory-side page tables coherent upon TLB shootdowns initiated by the CPU.  Our approach is similar to those used in integrated GPUs: an OS driver monitors any changes on virtual address spaces shared with MPUs, triggering update operations for the affected page table entries. Note that the inverted nature of the page tables eliminates any global coherence activity in the memory network as a virtual page maps to only one partition, and consequently, page table. Additionally, modifying the desired page table entry requires a single memory access in the common case, accounting for at most a few hundred nanoseconds. This additional overhead is not as significant as the TLB shootdown operation itself, which removes the stale entries in the TLBs of MPUs and CPU cores, and already takes tens of microseconds~\cite{oskin:software-managed}.\\

%\mjs{does this imply that all MPU translations are snooped into the CPU? discuss scalability?}

%\noindent\textbf{Cache hierarchy.} We assume that accelerators, much like conventional cores, could integrate te physical caches and an execution-side MMU with TLBs. Upon a page walk, the memory-side MMUs reply with the page table entry and cache block, which are stored in the MMU's TLB and data cache respectively. However, to avoid TLBs and TLB shootdowns~\cite{villavieja:didi}, we could use virtual caches. Recent practical designs for virtual cache hierarchies~\cite{yoon:revisiting, park:efficient} would be a perfect fit for SPARTA. In this approach, MPUs access the cache with virtual addresses, and upon a cache miss, the request is propagated to the memory-side MMUs to translate and fetch the corresponding block. The memory-side MMU only replies with the data cache block, simplifying our design.     

%\noindent\textbf{Synonyms.} In our current design, all the synonyms of a particular page frame need to map to the same memory set or partition. We believe this is not a significant limitation as it has been already included in commercial systems~\cite{cheng:virtual}. Nevertheless, our page table entries contain the whole page frame address, and hence with a slight modification in our design, we could enable synonyms to map anywhere. The only potential consequence is a drop in performance as a synonym page might map to a page frame residing in another memory partition. However, prior work has already shown that synonyms are both scarce and infrequent~\cite{yoon:revisiting, basu:reducing, park:efficient}, and therefore this overhead should be negligible.\\

%\noindent\textbf{DIPTA for CPUs.} DIPTA is a near-memory structure independent of any control flow, and any execution unit can use it to eliminate the translation overhead for the part of memory covered by DIPTA. While the focus of this work is on MPUs, CPUs can use DIPTA the same way MPUs do. However, CPUs may have to continue using TLBs in order to efficiently address any planar DDR chips and maintain full flexibility.\\

%\noindent\textbf{Multi-level memories.} Though prior work on MPUs assumes a single level~\cite{gao:practical, ahn:scalable, pugsley:ndc, ahn:pim-enabled}, memory can be organized as a hierarchy, with a die-stacked cache~\cite{reinders:knights, volos:fat} backed up by planar memory. For hardware-managed caches, the memory-side MMU performs the translation and accesses the partition, and in case of a cache miss, the page is fetched from planar memory as part of the standard cache miss operation. Once the page arrives into the partition, the data is sent back to the MPU. Note that moving the page from planar memory to the 3D memory does not affect the page table entry. In software-managed caches~\cite{reinders:knights}, MPUs rely on a software API for explicit migration of pages into the die-stacked memories.

%, as MPUs cannot access planar memory directly. 

%\noindent\textbf{Kernel memory.} We consider user instructions only as we argue that MPUs, like all prior custom hardware (e.g., GPU, FPGA), should execute only user code. Nevertheless, SPARTA is a great fit for the kernel, as Linux and FreeBSD's memory usage is almost entirely direct-mapped~\cite{mauerer:professional, mckusick:design} and memory resident. The TLB's tag matching logic would only require to skip the ASID bits for kernel accesses.

%As all the processes share the same kernel virtual addresses, the logic needs to ignore the ASID bits for kernel accesses. The implementation is trivial as Linux and FreeBSD partition the address space into two halves.

%, and hence the virtual address dictates whether to ignore the ASID bits.

%\mjs{does this imply that you want to run the kernel in the MPUs? i'm nto sure why this is an issue for your technique if only the CPU runs the kernel, all of its translations will just stay local and the MPUs will run their user-level code happily in the distance}

%\noindent\textbf{OS support.} The OS only needs to guarantee that the virtual page number and the page frame number map to the same memory set. OSs that support virtual caches already provide this capability (e.g., Solaris~\cite{cheng:virtual} and MIPS OS~\cite{taylor:tlb}). Therefore, the required modifications to OSs that do not have this feature should be feasible.




==> tex/evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}

\begin{figure*}
	\centering
	\subfloat[Memcached --- 1 Process]{
		\label{fig:memcached_1p}
		%  \includegraphics[width=.32\textwidth,clip,trim = 18mm 213mm 117mm 20mm]{figs/eps/sim-rread-lat.eps}}
		\includegraphics[width=.365\textwidth,clip]{graphs/memcached_assoc_1p-bw.pdf}}
	%  \hspace{.01in}
	\subfloat[RocksDB --- 1 Process]{
		\label{fig:rocksdb_1p}
		%  \includegraphics[width=.32\textwidth,clip,trim = 18mm 213mm 115mm 20mm]{figs/eps/sim-rread-bw.eps}}
		\includegraphics[width=.31\textwidth,clip]{graphs/rocksdb_assoc_1p-bw.pdf}}
	%   \hspace{.01in}
	\subfloat[Cassandra --- 1 Process]{
		\label{fig:cassandra_1p}
		%  \includegraphics[width=.32\textwidth,clip,trim = 28mm 217mm 115mm 20mm]{figs/eps/emu-rread-lat_cropped.eps}}
		\includegraphics[width=.31\textwidth,clip]{graphs/cassandra_assoc_1p-bw.pdf}}
	\caption{Overall miss ratio broken down into compulsory, capacity, and conflict misses.
		\label{fig:miss_ratio}}
\end{figure*}

%%%%%%%%%%% Table: Methodology %%%%%%%%%%%
\begin{table}
	\begin{center}
		\caption{Workload description.}
		\scalebox{0.7}
		\small
		\vspace{0.01in}
		\label{table:workload}
		\renewcommand{\arraystretch}{1.0}
		{\scriptsize
			\begin{tabular}{ l  l }
				%\hline
				\toprule
				{\bf Workload}                  & {\bf Description}  \\
				%\hline
				%\hline
				\toprule
				\multirow{1}{*}{Cassandra}                       &  NoSQL data store running Yahoo's YCSB. \\
				%\hline
				\cmidrule{2-2}
				\multirow{1}{*}{Memcached}                      & Cache store running Twitter-like workload~\cite{lim:thin}. \\
				%\hline
				\cmidrule{2-2}
				%\multirow{2}{*}{Core Types}    & In-order (Cortex A8-like): 2-wide \\
				%		                               &  OoO (Xeon-like): 4-wide, 128-entry ROB \\
				%\hline
				\multirow{1}{*}{TPC-H}	& TPC-H on MonetDB column store (Q1-Q21). \\
				\cmidrule{2-2}
				\multirow{1}{*}{TPC-DS}	& TPC-DS on MonetDB column store (Queries of~\cite{kocberber:meet}). \\
				\cmidrule{2-2}
				%\multirow{2}{*}{L1-I/D Caches}	&	32KB, split, 2 ports, 64B blocks, 10 MSHRs, \\
				%							& 2-cycle load-to-use latency \\
				\multirow{1}{*}{MySQL} 			& SQL DBMS running Facebook's LinkBench~\cite{facebook:linkbench}. \\
				%\hline
				\cmidrule{2-2}
				\multirow{1}{*}{RocksDB}                             &  Store engine running Facebook benchmarks~\cite{facebook:rocksdb}. \\ %a canonical uniform request distribution. \\
				%\hline
				
				\bottomrule
				%\hline
			\end{tabular}
		} %small
	\end{center}
	\vspace{-0.1in}
\end{table}
%%%%%%%%%%% END Table: Methodology %%%%%%%%%%%%

\begin{figure*}[t]
	\centering
	\subfloat[Memcached --- 2 Processes]{
		\label{fig:memcached_2p_assoc}
		\includegraphics[width=.36\textwidth,clip]{graphs/memcached_assoc_2p-bw.pdf}}
	\subfloat[Memcached --- 4 Processes]{
		\label{fig:memcached_4p_assoc}
		\includegraphics[width=.31\textwidth,clip]{graphs/memcached_assoc_4p-bw.pdf}}
	\subfloat[Memcached --- 8 Processes]{
		\label{fig:memcached_8p}
		\includegraphics[width=.31\textwidth,clip]{graphs/memcached_assoc_8p-bw.pdf}}
	\hspace{.01in}
	\subfloat[RocksDB --- 2 Processes]{
		\label{fig:rocksdb_2p}
		\includegraphics[width=.36\textwidth,clip]{graphs/rocksdb_assoc_2p-bw.pdf}}
	\subfloat[RocksDB --- 4 Processes]{
		\label{fig:rocksdb_4p}
		\includegraphics[width=.305\textwidth,clip]{graphs/rocksdb_assoc_4p-bw.pdf}}
	\subfloat[RocksDB --- 8 Processes]{
		\label{fig:rocksdb_8p}
		\includegraphics[width=.31\textwidth,clip]{graphs/rocksdb_assoc_8p-bw.pdf}}
	\hspace{.01in}
	\subfloat[Cassandra --- 2 Processes]{
		\label{fig:cassandra_2p}
		\includegraphics[width=.355\textwidth,clip]{graphs/cassandra_assoc_2p-bw.pdf}}
	\subfloat[Cassandra --- 4 Processes]{
		\label{fig:cassandra_4p}
		\includegraphics[width=.31\textwidth,clip]{graphs/cassandra_assoc_4p-bw.pdf}}
	\subfloat[Cassandra --- 8 Processes]{
		\label{fig:cassandra_8p}
		\includegraphics[width=.31\textwidth,clip]{graphs/cassandra_assoc_8p-bw.pdf}}
	
	
	\caption{Overall miss ratio broken down into compulsory, capacity, and conflict misses.
		\label{fig:miss_ratio_procs}}
\end{figure*}


%\javier{Points to come across:

%\begin{itemize}
%  \item Set-associativity doesn't increase page faults: 3C model %+ Memcached and RocksDB on real HW
%  \item TLB miss rate vs. working set for microkernels (hash %table, skip list, bst internal, bst external)
%  \item TLB miss penalty vs. working set (or sockets)
%  \item Fragmentation
%  \item $IPC =IPC_base + Penalty_tlb + Penalty_page_faults$
%\end{itemize}
%
%}


%\begin{figure*}[!h]
%\centering
% 
%  \subfloat[In-memory scenario.]{
%  \label{fig:speedup_memory_in}
%
%   \includegraphics[width=0.48\textwidth,clip]{graphs/speedup_inmemory.pdf}
%   }
%
%
%  \subfloat[Out-of-memory scenario.]{
%  \label{fig:speedup_memory_out}
%
% \includegraphics[width=0.48\textwidth,clip]{graphs/speedup_disk.pdf}
%  }



%\caption{Speedup over 4KB-H for 4KB-I, 2MB-H, 2MB-I, SPARTA, and an ideal translation.}
%  \label{fig:speedup_memory}
 
%\end{figure*}

%In this section, we perform a quantitative and qualitative study of the performance of different translation mechanisms.

We now perform a quantitative and qualitative study on VM.

\subsection{Performance Analysis}

The paper discusses many different workload scenarios and system configurations. As there are way too many performance points, we will show only the scenarios that have significant performance differences. First, we will show two workload scenarios, in-memory, where the memory size is equal to the working set size (i.e., the 1x ratio), and out-of-memory, where the working set size is eight times larger than the memory size (i.e., the 1/8x ratio). Second, as the performance across different process counts does not vary significantly, we are showing the average across runs. Third, the two topologies, daisy chain and mesh, behave similarly in terms performance, and hence we also present the average of both. Last, we present the results for different memory chip counts.

Fig.~\ref{fig:speedup_memory_in} shows the speedup of five translation mechanisms over the conventional MMU using 4KB pages and the hierarchical page table, labeled 4KB-H, for the in-memory scenario. The techniques are the conventional MMU using 4KB pages and the inverted page table, 2MB pages using the hierarchical and inverted page tables, SPARTA, and an ideal translation mechanism with zero translation overhead. We label the techniques as 4KB-I, 2MB-H, 2MB-I, SPARTA, and Ideal respectively. In the interest of space, we omit the results with 1GB pages, which perform better than 4KB pages but always worse than 2MB pages. The reason is that the number of entries in the MMU for 1GB pages is significantly limited, and server workloads have a large number of virtual segments which are accessed concurrently. First, we see that SPARTA clearly outperforms 4KB-H, 4KB-I, 2MB-H, and 2MB-I. In some cases by a large margin, up to $25\%$ for TPC-H. In other cases more moderately, $2.1\%$, $2\%$, $1.3\%$, and $0.5\%$ over 4KB-H, 4KB-I, 2MB-H, and 2MB-I respectively for MySQL. Most importantly, SPARTA is consistently on par with the ideal translation that incurs zero overhead for translation. Overall, SPARTA improves performance by $17.2\%$. $14\%$, $12.3\%$, and $10.5\%$ over 4KB-H, 4KB-I, 2MB-H, and 2MB-I respectively, and stays within 1.2\% of the ideal translation mechanism on average.

Fig.~\ref{fig:speedup_memory_out} presents the speedups for the out-of-memory scenario. As expected, the speedups are less significant that in the in-memory case. The reason is that all the cases incur the slowdown of resolving page faults, and therefore there are fewer accesses that can be accelerated. Still, SPARTA systematically performs better than the conventional MMU, $6.1\%$, $5.4\%$, $4.5\%$, and $4\%$ on average over 4KB-H, 4KB-I, 2MB-H, and 2MB-I respectively, and stays within 0.6\% of Ideal. 

Importantly, we model a greatly optimistic case when using $2$MB and $1$GB pages as we assume all pages are huge, with no generation overhead or fragmentation in any scenario. Additionally, we do not account for the excess in IO traffic generated by writing back dirty huge pages. Therefore, we expect further improvements with a realistic overhead. 

%Furthermore, we are conservatively assuming that all conflict page faults are major, and hence involve an access to secondary storage. Hence, in a real system, our speedups would likely be higher.


\subsection{Comparison with Other Proposals}

All the recent proposals on address translation for CPUs presented in Section~\ref{sec:uvm} aim to enhance the reach of TLBs by exploiting the contiguity available in the virtual and physical address spaces. Hence, these techniques are orthogonal to SPARTA as we reduce the TLB miss penalty. 

However, these techniques would be only effective for in-memory scenarios, and perform poorly for larger-than-memory working sets. In out-of-memory scenarios, direct segments~\cite{basu:efficient} would not be able to allocate the most frequently used pages in memory. Similarly, Redundant Memory Mappings and Hybrid TLB Coalescing~\cite{karakostas:redundant, park:hybrid} would not be able to allocate contiguous chunks of physical memory and fall back to base pages. CoLT~\cite{pham:colt} and Clustered TLBs ~\cite{pham:increasing} would also perform similar to the conventional translation when there is limited physical contiguity available. 

Even for in-memory scenarios, large address translation contiguity, on which proposed
TLB coalescing techniques rely~\cite{haria:devirtualizing,karakostas:redundant,gantz:hybrid,pham:colt,pham:increasing}, diminishes as the system runs. We adapt a representative kernel modification (increasing the max order of the buddy allocator), which enables large contiguous memory allocation (up to 1GB), to demonstrate the impact of memory fragmentation from long-run systems. We run a simple program \textit{mem\_sweep}, which allocates 30GB memory and accesses throughout all of it, along with our benchmarks back-to-back in our experimental machine with 32GB memory and measure the number of 1GB contiguous memory regions created by the modified kernel. Our program is able to obtain 28 of 1GB contiguous memory regions right after our experimental machine boots. The number decreases substantially to 8 at second round of execution and goes down to 5 (18\% of the number of 1GB contiguous memory regions at fresh boot time) after another 4 rounds of execution. The results show that memory fragmentation can significantly deter the contiguous memory creation, especially when the system's memory is fully utilized.


==> tex/float-translation-schemes.tex <==
\begin{figure}[h!]
\centering
 \subfloat[Baseline.]{
  \label{fig:baseline}
%  \includegraphics[width=.32\textwidth,clip,trim = 18mm 213mm 117mm 20mm]{figs/eps/sim-rread-lat.eps}}
   \includegraphics[clip,width=0.75\columnwidth]{figures/floorplan_vanilavm2.pdf}
%   \includegraphics[width=0.69\columnwidth]{figures/floorplan_vanilavm2.pdf}}
   }
%  \hspace{.01in}

 \subfloat[Per-Chip MMU.]{
  \label{fig:chipmmu}
%  \includegraphics[width=.32\textwidth,clip,trim = 18mm 213mm 115mm 20mm]{figs/eps/sim-rread-bw.eps}}
 \includegraphics[clip,width=0.75\columnwidth]{figures/floorplan_chipvm2.pdf}
 %  \includegraphics[width=0.69\columnwidth]{figures/floorplan_chipvm2.pdf}}
 }
% \hspace{.01in}

 \subfloat[Per-Partition MMU.]{
  \label{fig:partitionmmu}
%  \includegraphics[width=.32\textwidth,clip,trim = 18mm 213mm 115mm 20mm]{figs/eps/sim-rread-bw.eps}}
 \includegraphics[clip,width=0.75\columnwidth]{figures/floorplan_partitionvm2.pdf}
%  \includegraphics[width=0.695\columnwidth]{figures/floorplan_partitionvm2.pdf}}
 }

\caption{Different translation schemes on 4-chip floor plans. Large squares and small gray squares represent memory chips and partitions, respectively. Translation and memory access messages appear in blue and red, respectively. 
 \label{fig:translationSchemes_comparison}}
\end{figure}

==> tex/old-background.tex <==
\section{Background}
\label{sec:background}

\begin{figure}
	\centering
	\includegraphics[width=.85\columnwidth]{graphs/e2elatency-pattern.pdf}
	\caption{End-to-end latency of memory accesses.}
	\label{fig:e2elat}
\end{figure}


%\subsection{3D Memories}

\javier{Points to come across:

\begin{itemize}
  \item SW trend: Servers workloads are keeping their datasets memory resident; HW trend: Due to slowdown in silicon density and efficiency, computer system are integrating custom logic (accelerators).
  \item Explain the programmability benefits of pointer-is-a-pointer AND flexible VM system (e.g., demand paging, COW) of a conventional translation mechanism.
  \item TLB Reach Problem: Explain that a conventional translation mechanism is not effective for accelerators because (1) it relies on deep cache and TLB hierarchies and (2) data reuse, to bridge the gap between computation speed and memory capacity. However, accelerators primarily exploit parallel access with proximity to memory, and not reuse and deep cache hierarchies. Furthermore, accelerator are custom and hence silicon optimized, hence the available budget for translation hardware is limited. I think we can just cite prior work on TLB miss rates for in-memory workloads.   
  \item TLB Penalty Problem: Explain that compute and memory are scaling-out due to the slowdown in silicon scaling and efficiency, hence TLB misses (page walks) become more costly. We can show something similar to Figure 1 here.
\end{itemize}


}

%3D memory enables vertical stacks of multiple DRAM dies on top of a logic layer within a single package, leveraging low-latency/high-bandwidth through-silicon vias (TSVs). Two well-known incarnations of 3D memory technology are Micron's Hybrid Memory Cube (HMC)~\cite{hmc} and JEDEC's High Bandwidth Memory (HBM)~\cite{jedec:high}. Fig.~\ref{fig:overview}a illustrates the anatomy of a 3D memory chip. The chip consists of multiple vertical memory partitions, called vaults. Each vault is independent and similar to a conventional DDR channel, with its own DRAM controller and signals. Each DRAM controller connects to all the DRAM dies through a TSV bus. Similar to previous studies, MPUs are scattered across the vaults~\cite{ahn:scalable, gao:practical, pugsley:ndc, kim:neurocube}, while a network-on-chip (NoC) connects the vaults to each other and to the off-package links.

%Architectures that deploy 3D memories consist of a pool of CPUs and memory chips. Fig.s~\ref{fig:overview}b,~\ref{fig:overview}c,~and~\ref{fig:overview}d show the memory organizations considered in this paper. The CPU is connected to multiple memory chips using high-speed point-to-point SerDes links and a packet-based communication protocol. Fig.~\ref{fig:overview}b depicts a star topology where the CPU is connected to a small number of memory chips~\cite{fujitsu:while, reinders:knights}. Larger memory systems interconnect dozens of chips in a daisy chain (Fig.~\ref{fig:overview}c), which minimizes the number of links~\cite{gao:practical, pugsley:ndc}, or a mesh (Fig.~\ref{fig:overview}d), which minimizes the number of hops~\cite{ahn:scalable, kim:memory-centric}. 

%Memory accesses within the local partition are much cheaper than accesses to remote partitions, as the latter involves traversing expensive NoC and/or cross-chip interconnects. Fig.~\ref{fig:e2elat} compares the average end-to-end memory access latency depending on the target data's location: 1) same partition, 2) different partition, same chip, and 3) any chip in the network. The three cases are labeled as \textit{Partition}, \textit{Chip}, and \textit{Network} respectively. Unsurprisingly, the location of the data significantly affects latency. A data access in the local partition is the fastest; accessing a remote partition within the same chip is around $1.4\times$ slower, while accessing remote memory chips increases the latency by $3.5$--$10\times$, depending on the network and memory chip count. In summary, %these results indicate that optimizing for memory access latency requires MPUs to localize memory accesses within their partitions.

%\subsection{Unified Virtual Memory}
%\label{sec:uvm}

No prior proposal for virtually addressed MPUs is both general and efficient. The simplest approaches offload the address translation task to the CPU cores or an IOMMU~\cite{oskin:active, vesely:observation, gao:practical, xi:beyond}. Though simple, the fact that the MPUs and CPUs are on different chips means that sending translation requests to the CPU results in expensive chip-to-chip communication. Alternatively, one can integrate a traditional MMU with a TLB hierarchy per MPU. However, due to the limited reach of modern TLBs, page walks occur frequently, resulting in costly cross-chip traffic, as the multiple levels of the page table~\cite{gantz:hybrid} are arbitrarily scattered across the memory chips. All of these existing techniques create excessive cross-chip traffic, either to reach the CPU or to perform page walks, which could account for latencies of hundreds of nanoseconds, dramatically increasing the translation overhead.

Several recent proposals seek to improve the TLB reach. The most common approach is the introduction of larger page sizes~\cite{transparenthugepages, lighugetlbfs}. Similarly, CoLT~\cite{pham:colt} and Clustered TLBs~\cite{pham:increasing} coalesce 4-8 page translations into a single TLB entry, as long as their physical locations are contiguously in memory. Although the TLB reach improves, it is still unable to cover the entirety of a large memory system with tens or hundreds of GBs~\cite{gandhi:range}. More innovative ways of improving TLB coverage employ variable-size segments instead of fixed page-based translations~\cite{karakostas:redundant, park:hybrid, basu:efficient}. Unfortunately, the effectiveness of these techniques relies on the OS to allocate contiguous chunks of physical memory, which is not possible when the system is under memory pressure. Hence, page walks are still common in some scenarios, accounting for translation overheads of hundreds of nanoseconds. 

To summarize, there is no single approach capable of providing a unified VM that is suitable for all use cases. Prior work attempts to exploit contiguity in the physical memory, which is not always available. In contrast, our study focuses on sidestepping the need for fewer TLB misses by overlapping them with data fetch.








==> tex/old-intro.tex <==


%Advances in 3D integrated circuits are enabling systems with DRAM dies stacked on top of logic chips~\cite{hmc, diram, jedec:high}. These systems with custom memory processing units (MPUs) are projected to enable significant improvements in bandwidth, latency, and energy. Consequently, researchers have begun proposing MPUs for many types of computation~\cite{ahn:scalable, gao:practical, pugsley:ndc, kim:neurocube, xi:beyond, power:implications, mirzadeh:sort} and coined the term {\it near-memory processing} for this computation paradigm. %Along with the inclusion of 3D memories in industry products~\cite{fujitsu:while, reinders:knights}, there is substantial evidence suggesting that future systems may consist of a pool of CPU and MPU-capable memory chips.

\djordje{I think the main points that need to come across are:
(1) Server workloads keep more and more data in memory --> server memory grows sharply in capacity
(2) Both compute and memory are scaling out due to the diminished scaling. Compute gets specialized resulting in a huge number of small execution units/accelerators, often placed close to memory ->  Maximum (and average) distance between logic and memory keeps increasing, while the minimum distance keeps decreasing. 
(3) The effectiveness of hardware translation gets worse as memory grows (TLB reach), and as the distance between memory and logic grows (page walk latency). More complex hardware needed to keep up with growing memory. 
(4) Small accelerators have *the same or worse* translation hardware requirements as large CPU cores --> a) the hardware overhead of translation is huge relative to a tiny accelerator, b) the overall translation hardware in the system scales linearly with the number of accelerators.  
(5) The overhead of TLB coherence gets worse as the system grows (I'd rather leave it for another section)

The net results are that translation HW requirements grow with the number of accelerators AND with memory capacity, with its effectiveness getting worse with both. 

We propose a scalable mechanism whose whose effectiveness does not depend on memory size or number of accelerators, and whose hardware requirements will not grow with the number of accelerators.
}

\javier{I don't like Djordje's story because all the points can be easily addressed by DVM. We need to explain the tradeoff between translation HW and SW flexility and a table comparing all the previous approaches. For example, DVM shows 4 variables: programmability, power/perf, flexibility, and safety. I think a simple way to drive the message home is that you want both (1) the programmability benefits of pointer-is-a-pointer
AND (2) flexible VM system (e.g., demand paging, COW), which is essentially what conventional address translation gives you. Then, we explain why it doesn't work for accelerators and we continue with SpryVM.}


Large-scale IT services are increasingly run in memory to accommodate tight query latency requirements. Online services rely on larger memory capacity to keep data closer to processing logic and faster processing to improve cost/performance and return on investment. In light of the slowdown in silicon efficiency and density scaling in recent years, designers are resorting to hardware accelerators for a wide spectrum of applications ranging from deep learning \cite{}, to analytics\cite{} and graph processing \cite{}. 

%\begin{figure*}[t]
%	\centering
%	\includegraphics[width=0.85\textwidth]{figures/network.png}
%	\caption{Overview of a 3D memory architecture (a), and proposed and existing memory network topologies (b), (c), and (d).}
%	\label{fig:overview}
%\end{figure*}

%As with recent work on accelerators like GPUs~\cite{pichai:architectural, power:supporting}, a key research question is how virtual memory can be extended for MPUs. Enabling a unified virtual memory layer for CPUs and accelerators has many benefits: a simpler programming model, enabling "a pointer is a pointer everywhere" semantics~\cite{pichai:architectural, power:supporting, vesely:observation}, extending memory protection to accelerators, and obviating the need for manual inter-CPU-accelerator data marshalling. Vendors are already architecting unified virtual memory for GPUs (e.g., see AMD's Carrizo and Ryzen chips~\cite{wilcox:28nm}), with a view to generalizing it for all accelerators via the Heterogeneous System Architecture (HSA)~\cite{hsa}. Near-memory processing is following this integration path too~\cite{gao:practical, power:implications, xi:beyond}.

A salient feature of such accelerators is the need for a host CPU and OS to manage the execution resources among applications and application phases narrowing the scope of accelerator functionality to efficient and parallel in-memory computation. While many designers opt for accelerators to have direct physical access to memory, providing protection, isolation and the lack demand paging significantly complicates the software stack. Others have argued that the conventional virtual memory abstraction and a global address space programming model is best for software development enabling "a pointer is a pointer everywhere" semantics~\cite{pichai:architectural, power:supporting, vesely:observation}, extending memory protection to accelerators, and obviating the need for manual inter-CPU-accelerator data marshalling.


%Unfortunately, conventional virtual memory (VM) cannot simply be extended to MPUs without significant performance problems. The key culprit is virtual-to-physical address translation. Address translation performance is largely influenced by TLB capacity. As systems embrace ever-increasing memory sizes, it is difficult to design TLBs that provide adequate coverage of main memory. As a result, TLB misses are frequent, culminating in long-latency page table walks~\cite{pham:colt, pham:increasing, basu:efficient, karakostas:redundant, park:hybrid}. TLB overheads are known to be problematic for GPUs~\cite{pichai:architectural, power:supporting}, but we show that they are also detrimental to near-memory processing. Specifically, MPU TLB misses can be particularly long-latency because of the arbitrary distribution of page table entries across all the memory chips. Page table walks involve several chip-to-chip transfers of tens of nanoseconds per hop~\cite{huang:c3d, kanter:cavium, towles:unifying} for each level of the page table~\cite{gantz:hybrid}, incurring penalties of hundreds of nanoseconds. In other words, TLB overheads threaten to curtail the benefits of unified VM. 

Unfortunately, conventional virtual memory (VM) cannot simply be extended to accelerators. While general-purpose cores rely on deeper cache and TLB hierarchies and data reuse to bridge the gap between the core speed and memory capacity, accelerators primarily exploit parallel access with proximity to memory\cite{} forgoing reuse and deep hierarchies. The latter are also prohibitive in the required silicon resources relative to silicon-optimized accelerators. Moreover, accelerators are often designed to saturate the available memory bandwidth and are best placed near memory controllers, with physical memory partitioned among all accelerators to maximize parallelism\cite{}.


%The key culprit is virtual-to-physical address translation. Address translation performance is largely influenced by TLB capacity. As systems embrace ever-increasing memory sizes, it is difficult to design TLBs that provide adequate coverage of main memory. As a result, TLB misses are frequent, culminating in long-latency page table walks~\cite{pham:colt, pham:increasing, basu:efficient, karakostas:redundant, park:hybrid}. TLB overheads are known to be problematic for GPUs~\cite{pichai:architectural, power:supporting}, but we show that they are also detrimental to near-memory processing. Specifically, MPU TLB misses can be particularly long-latency because of the arbitrary distribution of page table entries across all the memory chips. Page table walks involve several chip-to-chip transfers of tens of nanoseconds per hop~\cite{huang:c3d, kanter:cavium, towles:unifying} for each level of the page table~\cite{gantz:hybrid}, incurring penalties of hundreds of nanoseconds. In other words, TLB overheads threaten to curtail the benefits of unified VM. Here we need to state that logic near memory can not afford deep TLB and cache hierarchies. Both the TLB reach and the page walk latency are key constraints.

Prior approaches to accommodate for accelerators either forgo VM and give direct physical access to memory for accelerators\cite{}, require major modifications to DRAM and memory controllers, or map physically contiguous regions of memory directly in VM or using segments\cite{}. These techniques fall short of providing the flexibility of a demand-paged VM and limit the utility of accelerators and/or introduce complex changes to the software stack.

%To address the problem, we observe that the main reason address translation impedes system performance is that it must complete before the subsequent data access. We take a back-to-basics approach and ask, is this serialization really necessary? In other words, is it possible to overlap memory translation with data fetch? By studying real-world server workloads, we identify that this decades-old serialized VM approach is an artifact of the early days of VM. In those days, memory was a scarce commodity and it was thereby necessary to enable a virtual page to map to any system page frame. This {\it fully associative} VM is flexible but requires memory translation to complete before data fetch.


In contrast, we propose {\it set-associative} VM, where a virtual page can map to one among a set of page frames. We dub this approach spryVM (Set-associative Page Regions of Your Virtual Memory). SpryVM restricts VM associativity so that a virtual address uniquely identifies the memory chip and partition that holds the data. This feature allows MPUs to access the memory as soon as the virtual address is known. Each memory partition integrates an MMU, which includes a TLB hierarchy and page table, that translates the virtual address and fetches the data---both the translation and data are always located in the MMU's local memory partition. SpryVM achieves low-overhead page walks as the page walk and data fetch operations overlap almost entirely. More specifically, our contributions are:

\noindent $\bullet$ A study of the VM associativity needs of modern server workloads. We are inspired by previous work on caches, which shows how associativity affects capacity, conflict, and compulsory misses \cite{hill:case}. 
We find that full VM associativity is often unnecessary, as most misses---page faults---are either compulsory or capacity, and are hence insensitive to associativity. Our study covers memory-resident and larger-than-memory working sets for single- and multi-programmed workloads.

%\item 
\noindent $\bullet$ A design space exploration for a hardware translation mechanism that leverages VM's modest associativity requirements. While such mechanisms do require OS changes, we show that these changes are readily-implementable as they can leverage existing and ongoing work on page coloring~\cite{mckusick:design}, multi-page table synchronization for heterogeneous memories~\cite{glisse:hmm}, and more. Moreover, we selectively apply set associativity to {\it regions} of the virtual address space that benefit from this approach. In so doing, we leave full-associativity for regions where it is better for performance, and retain cross-compatibility with existing systems.
%\item 

\noindent $\bullet$ SpryVM, a translation mechanism which restricts VM associativity so that a virtual address uniquely identifies a memory chip and partition, allowing MPUs to access the memory as soon as the virtual address is known. Each memory partition features an MMU, which includes a page table and TLB hierarchy to localize address translation and data fetch, thus minimizing the overhead. Each MMU's TLB hierarchy serves only its memory partition, makings its TLB performance robust across any memory chip and partition counts.

%\item 
\noindent $\bullet$ A comparison of spryVM with well-known translation mechanisms. SpryVM improves performance by up to $26\%$ and $15\%$ for in-memory and out-of-memory scenarios respectively, achieving almost-perfect zero-overhead address translation. 



Advances in 3D integrated circuits have enabled DRAM dies to be stacked on top of a logic chip~\cite{hmc, diram, jedec:high}. The projected benefits in bandwidth, latency, and energy have stimulated research and development of custom memory-side processing units (MPUs) on the logic chip for many different types of computation~\cite{ahn:scalable, gao:practical, pugsley:ndc, kim:neurocube, xi:beyond, power:implications, mirzadeh:sort}. Along with the inclusion of die-stacked memories in industry products~\cite{fujitsu:while, reinders:knights}, there is substantial evidence suggesting that future systems may consist of a pool of CPU and MPU-capable memory chips.


A key challenge in exploiting the full potential of these heterogeneous systems is the memory management between CPUs and MPUs. Industry initiatives such as the Heterogeneous System Architecture (HSA) Foundation are proposing to unify virtual memory (VM) between CPUs and any other processing unit in the system~\cite{hsa}. In this model, a pointer is equally valid on the CPU and MPU, simplifying data sharing and eliminating the need for explicit data copying and manual data consistency maintenance. In addition, VM enables efficient fine-grained memory accesses and transparent memory allocation and protection. Essentially, VM provides a familiar and powerful abstraction to programmers and operating systems alike. All these benefits have led HSA to adopt unified virtual memory into commercial GPUs, beginning with AMD's Carrizo chip~\cite{wilcox:28nm}. Given the benefits of HSA-style unified virtual memory and its early adoption and appearance in commercial products, we expect future computation units such as MPUs to also follow this integration path.

Unfortunately, the benefits of VM come at a significant performance overhead. Hardware support for address translation in commercial CPUs, which encompasses both per-core MMUs~\cite{intel:tlbs} and centralized IOMMUs for devices~\cite{intel:intel}, rely on TLB hierarchies that fall short of reaching the size of contemporary memories, resulting in frequent and long-latency page walks. Due to the arbitrary distribution of page table entries across all the memory chips, page walks involve several chip-to-chip transfers of tens of nanoseconds per hop~\cite{huang:c3d, kanter:cavium, towles:unifying} for each level of the page table~\cite{gantz:hybrid}, incurring in an unacceptable translation overhead of hundreds of nanoseconds. 

In this work, we observe that address translation stands on the critical path of accessing memory because a virtual page can map to any page frame---the mapping is fully associative. Hence, we perform an associativity study of VM (i.e., the number of locations that a virtual page can map to in the physical memory) across a variety of scenarios by classifying the page faults using the classic 3C model developed for caches~\cite{hill:aspects}. We conclude that capacity and compulsory misses---which are unaffected by associativity---dominate, while modest associativity is sufficient to eradicate conflict misses. More specifically, for working sets that are memory resident, compulsory misses dominate when the VM associativity equals the number of processes executing in the system. For working sets that exceed the memory size, capacity misses dominate and grow as a function of the working set size. In contrast, conflict misses become scarce once the associativity of virtual memory matches the number of processes in the system, and virtually disappear after the first few additional ways. Fundamentally, our associativity trends for VM match seminal work on set-associative caches~\cite{hill:aspects, cantin:cache}. 

We propose spryVM (Set-Associative Page Regions of your Virtual Memory), a VM system that restricts the associativity of VM so that a virtual address uniquely identifies a memory chip and partition. This feature allows MPUs to access the memory as soon as the virtual address is known. Each memory partition integrates an MMU, which includes a TLB hierarchy and page table, that translates the virtual address and fetches the data---both the translation and data are always located in the MMU's local memory partition. SpryVM achieves low-overhead page walks as the page walk and data fetch operations overlap almost entirely.

The primary contributions of this paper are:
%\begin{itemize}
%\item 

\noindent $\bullet$ A study of VM associativity using the 3C model. We show that full VM associativity is a largely unnecessary feature, as the majority of misses---page faults---are either compulsory or capacity, hence insensitive to associativity. Our study covers all scenarios: memory-resident and larger-than-memory working sets, single-process and multi-programmed. 

%\item 
\noindent $\bullet$ A design space exploration for a hardware translation mechanism that leverages VM's modest associativity requirements.
%\item 

\noindent $\bullet$ spryVM, a lightweight and high-performance translation mechanism which restricts VM associativity so that a virtual address uniquely identifies a memory chip and partition, allowing MPUs to access the memory as soon as the virtual address is known. Each memory partition features an MMU, which includes a page table and TLB hierarchy to localize address translation and data fetch, thus minimizing the overhead. 

%\item 
\noindent $\bullet$ An evaluation of spryVM against a set of state-of-the-art translation mechanisms. We show that our technique improves the performance of conventional address translation by up to $26\%$ and $15\%$ for in-memory and out-of-memory scenarios respectively, and almost eliminates the address translation overhead by performing within $1.2\%$ and $0.6\%$ of the ideal translation in each scenario respectively.
%\end{itemize}


While we propose using set-associative VM to tackle the address translation challenges posed by MPUs, our key observations are general and likely useful for broader classes of multi-chip systems. Set-associativity is a general concept applicable to any system with  a significant memory access latency due to expensive chip-to-chip traffic. For instance, one could also envision the ideas of set-associativity and co-location of data and translation within the same memory partition/chip being applied to classic multi-socket NUMA machines~\cite{hp:hp, huawei:kunlun, ning:open}. We hope our study will inspire researchers to leverage set-associativity in other multi-chip systems.



